Towards Misinformation Resilience in Pakistan: A Participatory Study with Low-Socioeconomic Status Adults

Digital misinformation disproportionately affects low-socioeconomic status (SES) populations. While interventions for the Global South exist, they often report limited success, particularly among marginalized communities. Through a three-phase participatory study with 41 low-SES Pakistani adults, we conducted formative interviews to understand their information practices, followed by co-design sessions that translated these user-identified needs into concrete design requirements. Our findings reveal a sophisticated moral economy of sharing and a layered ecology of trust that prioritizes communal welfare. These insights inform the Scaffolded Support Model, a user-derived framework integrating on-demand assistance with gradual, inoculation-based skill acquisition. We instantiated this model in our prototype, "Pehchaan," and conducted usability testing (N=15), which confirmed its strong acceptance and cultural resonance, validating our culturally grounded approach. Our work contributes a foundational empirical account of non-Western misinformation practices, a replicable participatory methodology for inclusive design, and actionable principles for building information resilience in resource-constrained contexts.

==> sections/limitations.tex <==
% % sections/limitations.tex
% \section{Limitations and Future Work}
% \label{sec:limitations}

% This study has several limitations that constrain the scope of our findings. As a qualitative inquiry, results may reflect self-censorship on sensitive political or religious topics, recall bias, and observer effects. Our co-design workshops engaged a relatively small sample, limiting diversity of captured perspectives, and we did not explicitly investigate gender dimensions of misinformation production and circulation. Our geographic focus on Pakistan constrains generalizability, though identified trust heuristics likely reflect broader South Asian contexts. Finally, our standalone application prototype reflects infrastructural constraints—while enabling novel design exploration, platform integration would offer greater usability and reach.

% Future work should pursue several directions to extend this foundation. Longitudinal deployments are needed to evaluate Pehchaan's sustained behavioral impact, assessing whether repeated engagement improves skepticism, detection accuracy, and user confidence. Larger evaluations across Pakistani regions would strengthen ecological validity and relevance for broader South Asian contexts. The Mashq Zone's pedagogical framework could advance from topical categories toward inoculation-based modules centered on manipulation techniques (impersonation, decontextualization, emotional appeals) with scaffolded progression from simple to sophisticated examples. Responsible development of AI components like Rehnumayi Chat requires robust fact-checking frameworks, bias safeguards, and moderation mechanisms. Finally, the HCI community should engage platform gatekeepers to advocate for APIs that enable the integration of community-centered intervention within high-traffic platforms where misinformation is actively circulated.
\section{Limitations and Future Work}
\label{sec:limitations}
This study has several limitations. Results may reflect self-censorship on sensitive political or religious topics, recall bias, and observer effects. Our co-design workshops engaged a relatively small sample, limiting diversity of perspectives, and we did not explicitly examine gender dimensions of misinformation. Our geographic focus on Pakistan constrains generalizability, though identified trust heuristics likely reflect broader South Asian contexts. Finally, our standalone prototype reflects infrastructural constraints—while enabling novel design exploration, platform integration would offer greater usability and reach.

Further research is needed. Quantitative and longitudinal studies are necessary to measure sustained behavioral impact and validate effectiveness at scale. Tracking engagement and shifts in information-sharing habits remains critical. Thus, the main contribution of this work is the Scaffolded Support Model, an architectural framework that, while developed for \textit{Pehchaan}, can inform efforts in other contexts.

Future work should extend this foundation through longitudinal deployments, larger evaluations across regions, and adaptation to other low-literacy, collectivist societies. Responsible development of AI components like Rehnumayi Chat requires fact-checking frameworks, bias safeguards, and moderation mechanisms. Finally, the HCI community should engage platform gatekeepers to integrate community-centered interventions within high-traffic platforms. Such efforts would further test the robustness of our framework and support globally inclusive strategies for information resilience.

